Robust Analytics for Video-Based Gait Biometrics

Gait analysis is the study of the systematic methods that assess and quantify animal locomotion. Gait finds a unique importance among the many state-of-the-art biometric systems since it does not require the subject's cooperation to the extent required by other modalities. Hence by nature, it is an unobtrusive biometric. This thesis discusses both hard and soft biometric characteristics of gait. It shows how to identify gender based on gait alone through the Posed-Based Voting scheme. It then describes improving gait recognition accuracy using Genetic Template Segmentation. Members of a wide population can be authenticated using Multiperson Signature Mapping. Finally, the mapping can be improved in a smaller population using Bayesian Thresholding. All methods proposed in this thesis have outperformed their existing state of the art with adequate experimentation and results.

==> Preamble/doc_prepend_A5.tex <==

%\newgeometry{tmargin=35mm,bmargin=30mm,lmargin=37mm,rmargin=37mm} % Added by Ebe

\pagestyle{fancy}
\fancyhf{}
\renewcommand{\headrulewidth}{0pt}
\renewcommand{\footrulewidth}{0pt}
\rhead{\thepage}
\rhead{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%------------------------Title page---------------------%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\hypersetup{
  pdfauthor={\@author},
  pdftitle={\@title},
  pdfsubject={PhD Thesis}
}
\let\Title\@title
\let\Author\@author
\let\Date\@date
\let\Fullname\@fullname
\makeatother

\begin{center}
  \LARGE
  \textbf{\MakeUppercase{\Title}} \\
  \vspace{1.5\baselineskip}
  \bigsize{\textbf{A THESIS}}\\
 \vspace{1\baselineskip}
  \normalsize{\textit{\textbf{Submitted by}}}\\
  \vspace{0.6\baselineskip}
  {\Large \textbf{\MakeUppercase{\Fullname}}}\\
  \vspace{1.6\baselineskip}
  \normalsize{\textit{\textbf{in partial fulfillment of the requirements for the degree of}}}\\
  %\normalsize{\textit{\textbf{of}}}\\
\vspace{.3\baselineskip}
  \bigsize{{\textbf{DOCTOR OF PHILOSOPHY}}}\\
\end{center}
\vspace{1\baselineskip}
  \begin{center}
   \includegraphics[width=26mm,height=25mm]{auemblem.pdf}   \\
  % \includegraphics[scale=0.4]{au-logo.png} \\
  \vspace{.3\baselineskip}
  \bigsize{\textbf{FACULTY OF INFORMATION AND }}\\
  \bigsize{\textbf{COMMUNICATION ENGINEERING}}\\
  \bigsize{\textbf{ANNA UNIVERSITY}}\\
  \bigsize{\textbf{CHENNAI  600 025}}\\ 
  \vspace{0.8\baselineskip}
  \large{\textbf{\MakeUppercase{\Date}}} % MAKE SURE YOU LOOK INTO THIS AT THE TIME OF SUBMISSION
 \end{center}
 \pagebreak

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%--------------------2nd and 3rd Page-------------------------%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \setboolean{@twoside}{false}
 \rhead{\thepage}
 {
\centering
\includegraphics[width=\linewidth]{Certificate.pdf}

\pagebreak
\includegraphics[width=\linewidth]{VivaProceedings.pdf}
}y
\pagebreak
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%--------------------Fourth Page-------------------------%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 
\rhead{\thepage}
\chapter*{ANNA UNIVERSITY\\
CHENNAI  600 025\\
\vspace{0.6\baselineskip}
CERTIFICATE}
\newlength{\aulength}
  \settowidth{\aulength}{Anna University
 Chennai}
\newlength{\datewidth}
\settowidth{\datewidth}{Chennai 600 025}
\begin{spacing}{1.8}
  \begin{sloppypar}
  \fontsize{13}{14.6}\selectfont 
    The research work embodied in the present
    thesis entitled ``\textbf{\MakeUppercase{\Title}}'' has been carried out in the
    Department of Computer Science and Engineering, Anna University,
    C.E.G. Campus, Chennai. The work reported herein is original and does not
    form part of any other thesis or dissertation on the basis of which a degree
    or award was conferred on an earlier occasion or to any other scholar.
    
    I understand the University's policy on plagiarism and declare that the
    thesis and publications are my own work, except where specifically
    acknowledged and has not been copied from other sources or been previously
    submitted for award or assessment.
  \end{sloppypar}
\end{spacing}

\newcommand*\leftright[2]{%
  \leavevmode
  \rlap{#1} %
  \hspace{0.6\linewidth}% Increase or decrease 0.5 to suit your needs. 
  #2}
  \begin{flushleft}
    \leftright{\textbf{\MakeUppercase{\Author}}}{\textbf{K. S. EASWARAKUMAR}} \\
    \leftright{RESEARCH SCHOLAR}{SUPERVISOR} \\
    \leftright{}{Professor} \\
    \leftright{}{Department of Computer}\\
    \leftright{}{Science and Engineering} \\
    \leftright{}{Anna University} \\
    \leftright{}{Chennai 600025.} 
  \end{flushleft}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%----------------Abstract and  ACK-----------------------%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  
\DeclareRobustCommand*{\tocheading}{%
    {{\normalfont\large\bfseries\centering CHAPTER NO. \hfill TITLE \hfill PAGE
        NO.\endgraf\bigskip}}}


\DeclareRobustCommand*{\toctabheading}{%
  {{\normalfont\large\bfseries\centering TABLE NO. \hfill TITLE \hfill PAGE
      NO.\endgraf\bigskip}}}
		
\DeclareRobustCommand*{\tocfigheading}{%
  {{\normalfont\large\bfseries\centering FIGURE NO. \hfill TITLE \hfill PAGE
      NO.\endgraf\bigskip}}}

                                  
\addtocontents{toc}{\protect\flushleft\protect\bfseries~CHAPTER
  NO.\hfill~TITLE\hfill~PAGE NO.\endgraf}
\addtocontents{toc}{\protect\flushleft \protect\bfseries
 ~ \hfill ~ \hfill ~\endgraf}

% \addtocontents{toc}{\protect\raggedleft Page\\}

\addtocontents{lof}{\protect\flushleft
\protect\bfseries FIGURE NO. \hfill
 TITLE \hfill  PAGE NO.\endgraf}%
\addtocontents{lot}{\protect\flushleft \protect\bfseries TABLE NO. \hfill
  TITLE \hfill  PAGE NO.\endgraf}%


\include{Main/abstract}
\include{Main/acknowledgement}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%----------------------- Contents -----------------------%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setlength\cftparskip{3pt}
\setlength{\cftbeforetoctitleskip}{-3em}
%\setlength{\cftaftertoctitleskip}{0 em}
\setlength{\cftbeforelottitleskip}{-3em}
\setlength{\cftbeforeloftitleskip}{-3em}
\cftsetindents{chapter}{15 mm}{10 mm}
\cftsetindents{section}{25 mm}{10 mm}
\cftsetindents{subsection}{35 mm}{12 mm} % 36 -> 35 edited by Ebe
\cftsetindents{subsubsection}{49 mm}{15 mm}
\cftsetindents{paragraph}{40 mm}{20 mm}
\cftsetindents{subparagraph}{50 mm} {20  mm}
\cftsetindents{table}{10 mm}{10 mm}
\cftsetindents{figure}{10 mm}{10 mm}
%\cftsecnumwidth=0pt
%\settocfeature{raggedhook}{\raggedright}

%%%%%%%% ADD TOC with one half spacing to TOC %%%%%%%%%%%

\newcommand*{\SetupNextPage}
  {\afterpage{\ifintoc\PrintChapterTocHeadline\fi}}
\begin{onehalfspacing}

  \begingroup
  % \let\cleardoublepage\clearpage
  \intoctrue
  \AtBeginShipout{\tocheading}
  \rhead{\thepage}
  %\rfoot{\includegraphics[width=13.7cm]{auresearchfooter.png}}
  % \setlength{\cftbeforechapskip}{1.5em} 
  \tableofcontents
  %\intocfalse
  \AtBeginShipoutClear
  \endgroup
  \newpage % it was \pagebreak

  \addcontentsline{toc}{section}{\bfseries LIST OF TABLES}
  \rhead{\thepage}
  %\rfoot{\includegraphics[width=13.7cm]{auresearchfooter.png}}
  \AtBeginShipout{\toctabheading}
  % \setlength\cftbeforechapskip{-0.5em}
  \listoftables
  \AtBeginShipoutClear
  \clearpage

  \rhead{\thepage}
  %\rfoot{\includegraphics[width=13.7cm]{auresearchfooter.png}}
  \addcontentsline{toc}{section}{\bfseries
    LIST OF FIGURES}
  \AtBeginShipout{\tocfigheading}
  \listoffigures
  \AtBeginShipoutClear
  %\clearpage
  %\endgroup
\end{onehalfspacing}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%----------------------- Acronyms -----------------------%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rhead{\thepage}
\fancyfoot[C]{\thepage}
%\rfoot{\includegraphics[width=13.7cm]{auresearchfooter.png}}

\include{Main/acronyms}


\clearpage
\newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%----------------------- Chapters -----------------------%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setboolean{@twoside}{true}


%\titleformat{\section}[hang]{\bfseries}{\makebox[20mm][l]{\thesection}}{0pt}{}{}
% \titleformat{\subsection}[hang]{\bfseries}{{\thesubsection}}{0pt}{}{}
% \titleformat{\subsubsection}[hang]{\normalsize\bfseries}{\makebox[20mm][l]{\thesubsubsection}}{0pt}{}{}
% \titleformat{\paragraph}[hang]{\normalsize\bfseries}{\makebox[20mm][l]{\theparagraph}}{0pt}{}{}
% \titleformat{\subparagraph}[hang]{\normalsize\bfseries}{\makebox[20mm][l]{\thesubparagraph}}{0pt}{}{}

% Added by Ebe to adjust the spacing before and after headings
\titlespacing\section{0pt}{0pt plus 0pt minus 2pt}{0pt plus 0pt minus 2pt}
\titlespacing\subsection{0pt}{0pt plus 0pt minus 2pt}{0pt plus 0pt minus 2pt}
\titlespacing\subsubsection{0pt}{0pt plus 0pt minus 2pt}{0pt plus 0pt minus 2pt}

\pagenumbering{arabic}
\pagestyle{fancy}
\fancyhf{}
\renewcommand{\headrulewidth}{0pt}
\renewcommand{\footrulewidth}{0pt}

\rhead{\thepage}

% Added by Ebe to make mirrored page numbering for twosided
\fancyhead{} % clear all fields
\fancyhead[LE,RO]{\thepage} %left header of even pages, number of the page. Right header of odd pages, number of the page

%\rhead{\thepage} % Comment if the one above is in use

%\fancyfoot[C]{\thepage}
\rfoot{\includegraphics[width=13.7cm]{auresearchfooter.png}}
\ausection

\sloppy
% \restoregeometry

\cleardoublepage
% Best place at the start of the Arabic numbered pages
% after \cleardoublepage and before the page number is
% reset in \pagenumbering{arabic}.
\pdfcatalog{%
  /PageLabels<<%
    /Nums[%
      % Page numbers are zero based.
      % Uppercase roman numbers starting with first page.
      0<</S/R>>%
      % Arabic numbers starting with current page.
      \the\numexpr\value{page}-1\relax<</S/D>>%
    ]%
  >>%
}
\pagenumbering{arabic}

\setlist[itemize]{topsep=0.0\parskip}


==> Preamble/pkg_and_fmt.tex <==
\renewcommand{\normalsize}{\fontsize{13 pt}{14.6 pt}\selectfont}

\makeatletter
\renewcommand{\@biblabel}[1]{\hfill#1.}
\def\@fullname{\relax}
\newcommand{\fullname}[1]{%
\gdef\@fullname{#1}}
\makeatother

%\setbiblabelwidth{50}
 \setlength{\labelwidth}{22.8pt}
 \setlength{\labelsep}{6.8pt}
 \setlength{\leftmargin}{0pt}
    %   \parsep\parskip
    \setlength{\itemsep}{1.3pt}
    \setlength{\topsep}{1.5pt}
  %\partopsep\parskip
    \itemindent\parindent
%   \advance\itemindent\labelsep
%\makeatother

%\usepackage{mathptm}

\usepackage{aunatbib} % Remove when the actual natbib is used
%\usepackage[sort,comma,numbers,authoryear]{natbib}
\usepackage{auapalike}
\usepackage{subfig}
\usepackage{bussproofs} % for deduction rules 
\usepackage{auphd}
\usepackage[toc]{glossaries}
\usepackage{array}
\usepackage{tabularx}
\usepackage[none]{hyphenat}
\usepackage{everypage}
\usepackage{changepage}
\newcounter{bibcount}
\newif\ifintoc
\makeatletter

\patchcmd{\@lbibitem}{\item[}{\item[\hfil\stepcounter{bibcount}{\thebibcount.}}{}{}
\setlength{\bibhang}{0\parindent}
\renewcommand\NAT@bibsetup%
  [1]{\setlength{\leftmargin}{\bibhang}\setlength{\itemindent}{-\parindent}%
\setlength{\itemsep}{\bibsep}\setlength{\parsep}{\z@}}

\makeatother
\usepackage{multirow}
\usepackage{multicol}
\usepackage{float}
\usepackage{booktabs} % For professional table layouts
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{latexsym}
\usepackage{verbatim}
\usepackage{ifthen}
\usepackage{graphicx}
\usepackage{epsfig}
\usepackage{pslatex}
\usepackage{setspace} % Fine-grained control over line spacing
\usepackage{titletoc}
\usepackage[subfigure]{tocloft}
\usepackage{longtable}
\usepackage{enumerate}
\usepackage{lscape} % To enable the temporary landscape environment
\usepackage{needspace} % To reserve some lines and thus to prevent page breaking for those lines.
\usepackage{enumitem}
\usepackage[chapter]{algorithm} 
%\usepackage{algorithmic}  
%\usepackage[ruled]{algorithm2e}
\usepackage{atbegshi}
\usepackage[nobottomtitles*]{titlesec} % nobottomtitles option added by Ebe (but can still occur)
 

% Packages listed by Ebe
\usepackage{algpseudocode}
\usepackage{textcase}
\usepackage{csvsimple}
\usepackage{gensymb} % Degree symbol
\usepackage[tmargin=35mm,bmargin=30mm,lmargin=25mm,rmargin=25mm, bindingoffset=10mm]{geometry}
\usepackage{hyperref}
%\usepackage{showframe} % Shows the margin outlines for checking (not for printing)

\author{Ebenezer R.H.P. Isaac}

% Convenience macro by Ebe
\newcommand{\tabitem}{\par\hspace*{\labelsep}\textbullet\hspace*{\labelsep}\hangindent=6mm}
\newcommand\peq{\mkern1.7mu{=}\mkern1.7mu}


\usepackage{makeidx}
\newenvironment{pf}{{\vspace{-18pt}\noindent\textbf{Proof.}}}{\hfill {\fbox{}}}
\newtheorem{defi}{Definition} [chapter]
\newtheorem{prop}{Property} [chapter]
\newtheorem{props}{Proposition}
\newtheorem{conject}{Conjecture}
%\theoremstyle{plain}
\newtheorem{lemma}{Lemma} [chapter]
\newtheorem{theo}{Theorem}[chapter]
\newtheorem{ex}{Example} [chapter]
\usepackage[format=hang,labelfont=bf,textfont=bf]{caption}
\captionsetup[algorithm]{labelsep=colon} % Added by Ebe

\PassOptionsToPackage{linktocpage}{hyperref}
\tocloftpagestyle{myheadings}
\usepackage{tocloft}% http://ctan.org/pkg/tocloft
\usepackage{atbegshi}
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\let\PBS=\PreserveBackslash
\makenoidxglossaries
\printnoidxglossaries
  \usepackage{afterpage}
\usepackage{colortbl}
\usepackage{newlfont}
%\loadglsentries{glossary}
\newboolean{psoutput}
\setboolean{psoutput}{true}
\usepackage{pst-all}
\newcommand{\defname}[1]{\emph{#1}.}
\newtheorem{fact}{Fact}[chapter]
\floatstyle{ruled}
\newfloat{algorithm}{htp}{loa}
\floatname{algorithm}{Algorithm}
 \newcounter {definition}[chapter]
\renewcommand \thedefinition {\arabic{chapter}.\arabic{definition}}
\newenvironment{definition}
{ \refstepcounter{definition}
   {\noindent \bf Definition \arabic{chapter}.\arabic{definition}.}}
 {}
 \def\enddefinition{$\Box$}

 \newcounter {example}[chapter]
 \renewcommand \theexample
 {\arabic{chapter}.\arabic{example}}
 \newenvironment{example}
 { \refstepcounter{example}
   {\noindent \bf Example \arabic{chapter}.\arabic{example}.}}
 {}
 \def\endexample{$\Box$}

 \newcounter {proposition}[chapter]
 \renewcommand \theproposition {\arabic{chapter}.\arabic{proposition}}
 \newenvironment{proposition}
 {\refstepcounter{proposition}
   {\noindent \bf Proposition \arabic{chapter}.\arabic{proposition}. }}
 {}
 \def\endproposition{$\Box$}

\pagenumbering{roman}
\setcounter{page}{1}
\setcounter{secnumdepth}{6}
\setcounter{tocdepth}{6}
\renewcommand{\baselinestretch}{1.5}
\newcommand{\row}{i}
\newcommand {\combined} {{C}}
\newcommand {\mtis} {}

\newboolean{showalter}
\setboolean{showalter}{true}
\newcommand{\alter}[1]{\ifthenelse{\boolean{showalter}}{ \{ #1 \} }{}}
\providecommand{\tabularnewline}{\\}
\newcommand{\bigsize}{\fontsize{15pt}{20pt}\selectfont}

\renewcommand{\cfttoctitlefont}{\bfseries\Large}
\renewcommand{\cftlottitlefont}{\bfseries\Large}
\renewcommand{\cftloftitlefont}{\bfseries\Large}


\makeatletter
\renewcommand{\@dotsep}{10}
\newcommand{\AtBeginShipoutClear}{\gdef\AtBegShi@Hook{}}
\makeatother
\renewcommand{\cftdot}{ }
\cftsetrmarg{1.5in} % changed by bama - earlier it was 1.5 inch. right margin is decreased to 1 inch.
\setlength{\parskip}{3.5ex plus 0ex minus 0ex }
\setlength{\textfloatsep}{10mm plus 2mm minus 2mm}
%\setlength{\parfillskip}{3.6ex}

% \widowpenalties=3 10000 10000 15 0
% \clubpenalties=3 10000 10000 15 0
\widowpenalty=10000 % changed by Ebe
\clubpenalty=10000

\usepackage{fancyhdr}
\AtBeginDocument{\addtocontents{toc}{\protect\thispagestyle{fancy}}} 
\AtBeginDocument{\addtocontents{lof}{\protect\thispagestyle{fancy}}} 
\AtBeginDocument{\addtocontents{lot}{\protect\thispagestyle{fancy}}} 
\setlength{\footskip}{50pt}

%\setcitestyle{aysep={}} % activate when natbib is in use
%\settocfeature{raggedhook}{\raggedright}



